Defining Requirements Strategies in Agile: A Design Science Research Study

Research shows that many of the challenges currently encountered with agile development are related to requirements engineering. Based on design science research, this paper investigates critical challenges that arise in agile development from an undefined requirements strategy. We explore potential ways to address these challenges and synthesize the key building blocks of requirements strategies. Our design science research rests on a multiple case study with three industrial cases in the domains of communication technology, security services, and automotive. We relied on a total of 20 interviews, two workshops, participant observation in two cases, and document analysis in each of the cases to understand concrete challenges and workflows. In each case, we define a requirements strategy in collaboration with process managers and experienced engineers. From this experience, we extract guidelines for defining requirements strategies in agile development.

==> 6-discussion.tex <==
\section{Discussion}

%\eric{The following text might be shortened a bit and used as conclusion.}
 
The significant contribution of this design cycle study is to define the term “requirements strategy.”


Requirements strategy, defined for each challenge, can be applied to any company facing similar challenges. Also, agile companies can establish their requirements strategy according to their challenges utilizing their defined baseline values. 
 
 
%\subsection{Implications to Research}


%\eric{RE is often perceived as a inherently plan-driven activity, corresponding to a waterfall phase. Also, with a focus on documentation, it is not a good fit for agile.}

\paragraph{RE is not a good fit for agile}
RE is often perceived as an inherently plan-driven activity. It focuses on eliciting user needs and desires and formulating the agreed-upon set of requirements which provides the basis for subsequent development activities. Furthermore, it heavily focuses on docume\cite{leffingwell2000managing}. However, it contradicts the agile manifesto and does not fit agile development methodologies \cite{kasauli2021requirements}.


{By \ins{relying on the theory of shared understanding, we} \chg{embracing}{embrace} RE as a knowledge management problem\chg{, we}{and} create a RE strategy model that allows to focus on aspects that are independent of documentation and waterfall phases.}

Our findings therefore allow discussing RE activities in an agile context, without getting lost in discussing extensive methodologies, or even method engineering, which often don't yield good results in an agile context.

\paragraph{RE strategy to resolve RE knowledge management problem }

By embracing RE as a knowledge management problem \cite{serna2018framework}, we create a RE strategy model that allows focusing on aspects that are independent of documentation and waterfall phases. Our findings, therefore, allow discussing RE activities in an agile context without getting lost in discussing extensive methodologies, which often do not yield good results in an agile context.
Instead, we hope that our contribution allows to focus on what creates value in an agile context, and in this way enables future research, especially currently slowed down by reluctance of agile methods to incorporate requirements engineering methodology.

%\eric{Instead, we hope that our contribution allows to focus on what creates value in an agile context, and in this way enables future research, especially currently slowed down by reluctance of agile methods to incorporate requirements engineering methodology.}


%\eric{Focus on what brings value to agile (also in terms of RE research) and highlight three important perspectives to consider (see Table II).}

\ugh{Agile development allows for frequent customer feedback and the correct requirements with the proper emphasis on them. However, it is challenging to maintain frequent feedback to the right persons or roles in large-scale agile. These challenges create barriers to identifying and building a shared understanding of customer values. So our proposed strategy improvise to mitigate the identified challenges. Particularly considering these following perspectives, i.e., structural, organizational, and work and feature flow perspectives, see table \ref{tab:strategy-perspectives}.}


\eric{relate to situational method engineering (BPM often does not work well in agile contexts, our re strategy provides a more lightweight tool for this purpose.)}

\ins{Our requirements strategy can be interpreted of an instance of situational method engineering \cite{henderson2010situational} where we focus on the context of agile system development and requirements methods in particular. By this, we aim to make it easier for practitioners to integrate RE in their agile workflows.}

\eric{We hope to encourage future research on...}

%\subsection{Implications to Practice}

%Based on the literature and our case studies, we formulated the following implications to practice for applying requirements in agile development in large scale organizations.


%\paragraph{Requirements communication} 
%Information related to a requirement, such as why it is needed or what is the associated customer value, falls in the category of implicit knowledge. Implicit knowledge is usually based on assumptions; and thus easily trips away after meetings, particularly in agile development. There is even a high risk of loss of implicit information in large-scale agile, where we have a long communication chain and information is not shared to the end of the chain. Thus to have a good shared understanding of requirements, we need to ensure that all the requirements-related information is properly communicated.

%\paragraph{Just enough Documentation.} Documentation is necessary to record the information for communication reusability and to make some implicit information explicit. Just enough documentation means that documentation should be large enough to have all the necessary information to transfer knowledge( but not the details) and small enough for the maintenance of documentation. Particularly in large scale organizations, where we have many teams, they cannot communicate face-to-face with each other, or to save this communication time wastage, just enough documentation is necessary. Case 3 is already working on this but is still not mature in practice. 

%\paragraph{Need to setup tools and practices}The requirements engineering strategy model focuses on organizations' tools and practices to strategically handle the requirements engineering problems. For instance, the RE strategy focuses on regularly reviewing and updating customer requirements to avoid many internal problems, e.g., avoiding decentralized requirements and addressing customer involvement problems. Similarly, we need to set up the tools that allow developers to own requirements. 




 



